Generate, Discriminate and Contrast: A Semi-Supervised Sentence Representation Learning Framework

Most sentence embedding techniques heavily rely on expensive human-annotated sentence pairs as the supervised signals. Despite the use of large-scale unlabeled data, the performance of unsupervised methods typically lags far behind that of the supervised counterparts in most downstream tasks. In this work, we propose a semi-supervised sentence embedding framework, GenSE, that effectively leverages large-scale unlabeled data. Our method include three parts: 1) Generate: A generator/discriminator model is jointly trained to synthesize sentence pairs from open-domain unlabeled corpus; 2) Discriminate: Noisy sentence pairs are filtered out by the discriminator to acquire high-quality positive and negative sentence pairs; 3) Contrast: A prompt-based contrastive approach is presented for sentence representation learning with both annotated and synthesized data. Comprehensive experiments show that GenSE achieves an average correlation score of 85.19 on the STS datasets and consistent performance improvement on four domain adaptation tasks, significantly surpassing the state-of-the-art methods and convincingly corroborating its effectiveness and generalization ability.Code, Synthetic data and Models available at https://github.com/MatthewCYM/GenSE.

==> tables/gen_samples.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{l|l|l}
\toprule
\textbf{Method}       & \textbf{Entailment}    & \textbf{Contradiction}     \\
\midrule
& \multicolumn{2}{l}{\textit{\textbf{Input:} A young man getting ready to release a red kite.}}  \\
\midrule
DINO & A young man releasing a red kite. & A man getting ready to release a red kite. \\
\midrule
Retrieval & A man getting ready to fly a kite.                & N/A \\
\midrule
BackTrans & A young man prepares to release a red kite.       & N/A \\
\midrule
GenSE     & The man is prepared to fly the kite.  & A man is playing basketball. \\
\bottomrule
\end{tabular}


\caption{Comparison of different data synthesis approaches. For retrieval and back-translation, only entailment pairs can be obtained. More samples are presented in appendix}
\label{tab:gen_samples}
\end{table*}
